TP-Aware Dequantization

In this paper, we present a novel method that reduces model inference latency during distributed deployment of Large Language Models (LLMs). Our contribution is an optimized inference deployment scheme that address the current limitations of state-of-the-art quantization kernels when used in conjunction with Tensor Parallel (TP). Our method preserves data locality in GPU memory access patterns and exploits a priori knowledge of TP to reduce global communication. We demonstrate an up to 1.81x speedup over existing methods for Llama-70B and up to 1.78x speedup for IBM WatsonX's Granite-20B MLP layer problem sizes on A100 and H100 NVIDIA DGX Systems for a variety of TP settings.

==> equations/general_tp_aware_method.tex <==
\begin{algorithm}[H]
\caption{General TP-aware Algorithm}
\label{alg:optimized_matmul}
\begin{algorithmic}[1]
\Require $A_{\text{N-1}}, W_{\text{N-1}}, W_{\text{N}}$ 
\Require $P_{\text{N-1}}, P_{\text{N}}$ 
\State $A_{\text{N}} \gets A_{\text{N-1}}[:, P_{\text{N-1}}] \ @ \ W_{\text{N-1}}[P_{\text{N-1}}, P_{\text{N}}]$
\State $Y_{\text{N}} \gets A_{\text{N}} \ @ \ W_{\text{N}}[P_{\text{N}}]$
\State \Return $Y_{\text{N}}$
\end{algorithmic}
\end{algorithm}




==> figures/matrix_multiply.tex <==
\begin{figure}[H]
\centering
\begin{adjustbox}{center}
\begin{tikzpicture}[>=Stealth]
    % Matrix A1
    \matrix (A1) [matrix of math nodes,left delimiter={[},right delimiter={]}] {
        a_{12} & a_{11} & \cdots \\
        a_{22} & a_{21} & \cdots \\
        \vdots & \vdots & \ddots \\
    };
    \node [above=0.5cm of A1] (labelA1) {$A1$};

    % Permutation Matrix P1 
    \node [right=2cm of A1, draw, minimum size=1cm, regular polygon, regular polygon sides=6] (P1) {$P1$};
    \node [above=0.5cm of P1] (labelP1) {permute $P_{\text{N-1}$};

    % Matrix W1
    \matrix (W1) [matrix of math nodes,right=2cm of P1,left delimiter={[},right delimiter={]}] {
        w_{22} & w_{21} & \cdots \\
        w_{12} & w_{11} & \cdots \\
        \vdots & \vdots & \ddots \\
    };
    \node [above=0.5cm of W1] (labelW1) {$W1$};

    % Permutation Matrix P2 (perm2)
    \node [right=2cm of W1, draw, minimum size=1cm, regular polygon, regular polygon sides=6] (P2) {$P2$};
    \node [above=0.5cm of P2] (labelP2) {permute $P_{\text{N}$};

    % Matrix W2
    \matrix (W2) [matrix of math nodes,right=2cm of P2,left delimiter={[},right delimiter={]}] {
        w_{21} & w_{22} & \cdots \\
        w_{11} & w_{12} & \cdots \\
        \vdots & \vdots & \ddots \\
    };
    \node [above=0.5cm of W2] (labelW2) {$W2$};

    % Arrows
    \draw[->] (A1) -- (P1);
    \draw[->] (P1) -- (W1);
    \draw[->] (W1) -- (P2);
    \draw[->] (P2) -- (W2);

    % Resulting Matrix
    \matrix (R) [matrix of math nodes,below=2cm of W1,left delimiter={[},right delimiter={]}] {
        r_{11} & r_{12} & \cdots \\
        r_{21} & r_{22} & \cdots \\
        \vdots & \vdots & \ddots \\
    };
    \node [below=0.1cm of R] (labelR) {Result};

    % Arrows to Result
    % \draw[->] (W1) -- (R);
    \draw[->] (W2) |- (R);


    % Labels for operations
    \node [below=0.5cm of P1] (op1) {1. $A_{\text{N}} = A_{\text{N-1}}[:, P_{\text{N-1}}] \ @ \ W_{\text{N-1}}[P_{\text{N-1}}, P_{\text{N}}]$};
    \node [below=0.5cm of P2] (op2) {2. $Y_{\text{N}} = A_{\text{N}}[:, P_{\text{N-1}}] \ @ \ W_{\text{N}}[P_{\text{N}}]$};
    \node [below=0.5cm of R] (op3) {3. $Y_{\text{N}} = A_{\text{N}} \ @ \ W_{\text{N}}[P_{\text{N}}]$};

    
\end{tikzpicture}
\end{adjustbox}
\caption{Illustration of TP-aware Method}
\label{fig:matrix_operations_optimized}
\end{figure}
